Deep Parametric Continuous Convolutional Neural Networks

Standard convolutional neural networks assume a grid structured input is available and exploit discrete convolutions as their fundamental building blocks. This limits their applicability to many real-world applications. In this paper we propose Parametric Continuous Convolution, a new learnable operator that operates over non-grid structured data. The key idea is to exploit parameterized kernel functions that span the full continuous vector space. This generalization allows us to learn over arbitrary data structures as long as their support relationship is computable. Our experiments show significant improvement over the state-of-the-art in point cloud segmentation of indoor and outdoor scenes, and lidar motion estimation of driving scenes.

==> background.tex <==
\section{A Review on Convolution Operators \raquel{convolution or convolutional?}}
In this section we provide a review  on  convolution operators  over discrete and continuous domain. 
Convolution is a mathematical operator over two functions  $f$ and $g$, which produces a third function $h$. 

\begin{figure}
  \includegraphics[width=1.02\linewidth]{figs/continuous_conv.pdf}
  \caption{Standard Grid Convolution vs. Continuous Convolution. In grid convolution 3x3 kernel function in grid convolution could only takes 9 possible values as input. And despite image boundaries, input and output are corresponding to the same points in the domain. In continuous convolution, kernel function takes arbitrary point in continuous domain as input, and it is possible to output features at the point that was not seen in the input.  } 
  \label{fig:idea}
\end{figure}

\paragraph{Generic Convolution over Groups:}
Considering a subset $\mathcal{S}$ in a group $\mathcal{G}$, with  mutually inverse operators   $+$ and $-$  defined in the group $\mathcal{G}$. %
\raquel{do we need to define what mutually inverse is? shouldnt you first define the group and its operations and then the subgroup} Note that $\mathcal{S}$ does not necessarily have closure under $+$ and $-$ operators. Given two functions $f$ and $g$ defined on $\mathcal{G}$, the convolution filter can be defined as: 
\begin{equation}
\label{conti-conv}
h(\bx) = \sum_{\by \in \mathcal{S}} f(\by) g(\by - \bx)
\end{equation}
 Especially there are two special cases that are worth to be discussed: 
\paragraph{Continuous Convolution:}
Let $f$ and $g$ be functions over the real-valued domain, \ie $\mathcal{G} = \mathcal{S} = \mathbb{R}$.  The convolution operator is then defined as the following integral %
\begin{equation}
\label{conti-conv}
h(\bx) = (f \ast g) (\bx) = \int_{-\infty}^{\infty} f(\by) g(\by -\bx) d\bx
\end{equation}
where $h(t)$ can be described as a weighted average of the function $f$ around the point $t$, where the weight is given by $g(-\tau)$ shifted by $t$. 

\paragraph{Discrete Convolution:}
Let  $f$ and $g$ be functions defined over the support domain of finite integer set: $\mathcal{G} = \mathcal{Z}^D$ and $ \mathcal{S} = \{ -M, -M + 1, ..., M - 1, M\}^D$, the convolution operator between $f$ and $g$ is defined as: 
\[
h[n] = (f \ast g)[n] = \sum_{m = -M}^M f[n - m] g[m] 
\]
Note that if $D = 2$ we recover  the standard convolution operator over 2D images. And if $D = 3$ we recover the standard convolution operator conducted on 3D volumetric representations. Due to the finite state in the support domain, one convolution kernel $g$ can be parameterized by $(M+1)^2$ real-values. 
